An Arithmetic Theory for the Poly-Time Random Functions

We introduce a new bounded theory RS^1_2 and show that the functions which are Sigma^b_1-representable in it are precisely random functions which can be computed in polynomial time. Concretely, we pass through a class of oracle functions over string, called POR, together with the theory of arithmetic RS^1_2. Then, we show that functions computed by poly-time PTMs are arithmetically characterized by a class of probabilistic bounded formulas.

==> Buss.tex <==
% !TEX root = main.tex


 
Arithmetic theories are related to computable functions
in several ways. 
%
In the 1970s-80s, 
also fragments of $\PA$ started to receive attention.
%
Indeed, these sub-theories not only 
support a satisfactory axiomatization –
somehow escaping proof-theoretical drawbacks coming
from incompleteness~\cite{Godel} – but are also
deeply connected with interesting complexity classes~\cite{Parikh,CookReckhow}.
%
In particular, in 1986 Buss introduced a bounded theories of arithmetic 
able to characterize the class of \emph{poly-time} computable function~\cite{Buss86}.
%
Inspired by this work, also Ferreira defined a theory 
equivalent to the corresponding one by Buss, but expressed
in a \emph{word language}, and corresponding to the
class of poly-time functions \emph{over strings}~\cite{Ferreira90}.
%
%
%
%
%
\small
%
\begin{center}
 \begin{figure}[h!]
\framebox{
\parbox[t][4.5cm]{12cm}{
\begin{center}
\begin{chronology}[25]{1885}{2005}{\textwidth}
\event[1889]{1889}{Peano Arithmetic (1889)} %~\cite{Peano}}
%
\event[1950]{1950}{Robinson $\textbf{\textsf{Q}}$ (1950)} %~\cite{Robinson}}
%
\event[1971]{1971}{Parikh's $\textsf{\textbf{I}}\Delta_0$ (1971)} %~\cite{Parikh}}
%
\event[1984]{1984}{Buss' Bounded Arithmetic (1986)} %~\cite{Buss86}}
%
\event[1990]{1990}{Ferreira's $\Sigma^b_1$-NIA (1988/90)} %~\cite{Ferreira90}}
\end{chronology}
\end{center}
%
 }}
\caption{From Peano to Bounded Arithmetics}
\end{figure} 
\end{center}


\normalsize




%%%%%% SUB-THEORIES OF ARITHMETIC AND COMPLEXITY
\subsection{Sub-Theories of Arithmetic and Complexity}

\paragraph{Very Weak, Weak and Strong Fragments.}
Sub-theories of $\PA$ have been obtaining
increasing interest for their intimate connection with 
complexity classes.
%
%Differently from $\PA$, these theories can support satisfactory axiomatizations, somehow  escaping proof theoretical drawbacks of incompleteness~\cite{Godel}.
%
Buss divided them into three main categories:
strong, weak and very weak fragments~\cite{Buss98}.
%
\emph{Very weak} theories do not admit any induction axioms.
%
Among them there is well-known Robinson arithmetic 
$\textsf{\textbf{Q}}$, introduced in the 1950s by Robinson, Tarski, and Mostowski~\cite{Robinson,TarskiMostowskiRobinson}.
%\footnote{$\PA$ can be seen as obtained by adding to $\textsf{\textbf{Q}}$ the induction schema for any first-order formula.}
%
\emph{Weak theories} are defined by a language which
extends that of $\PA$ by additional symbols of specific
growth rate (sometimes together with explicit bounded quantifiers) and
by limited induction schemas.
%
In \emph{strong theories} the language 
is enlarged so to include symbols for all primitive
recursive functions.\footnote{Examples of strong theories
are $\textsf{\textbf{I}}\Sigma_n$, that is 
$\textsf{\textbf{Q}}_\leq$ (the conservative extension
of $\textsf{\textbf{Q}}$ with $x \leq y \leftrightarrow
(\exists z)(x+z=y)$) plus $\Sigma_n$-IND, and
$\textsf{\textbf{I}}\Delta$ obtained adding $\Delta_0$-IND to $\textsf{\textbf{Q}}_\leq$.}





\paragraph{Bounded Theories.}
In particular, bounded theories of arithmetics
are weak fragments of $\PA$,
typically including bounded quantifiers
and in which induction is limited.
%
Buss defined a bounded arithmetic as a theory
axiomatized by $\Pi_1$-formulas~\cite{Buss98}.
%
%As said, one of the main motivations for studying $\BA$ is the connection to low-level complexity and, in particular, the relation with $\PH$.
%
The potential strength of such theories 
and their ability to characterize complexity, 
depends on the (sub-exponential) 
growth rate of the function symbols in the language.
%Usually $\BA$ includes only functions of sub-exponential growth rate including $\omega_1$ and $\#$.
%
%Generally speaking, these theories were introduced to characterize standard complexity classes.
%
The study of $\BA$ was initiated by Parikh in 1971~\cite{Parikh},
who introduced $\textsf{\textbf{I}}\Delta_0$ to give an appropriate
proof theory to linear bounded automata, namely to predicates
computable by linear space-bounded TMs.
%
Then, other bounded theories were introduced by Buss~\cite{Buss86}
and 
extensively studied.
%The other, was introduced by Buss~\cite{Buss86}. Cook also introduced an equational theory  $\textsf{\textbf{PV}}$ (polynomially verifiable) formalizing feasibly constructive proofs, that is poly-time reasoning.










%%%%%% BUSS BOUNDED ARITHMETIC
\subsection{Buss' Bounded Arithmetic}
Buss' Ph.D. thesis~\cite{Buss86} provided a groundbreaking result
in the study of the arithmetical characterization of complexity classes.
%
He started by considering the \emph{definability}
of a function in a theory: an arithmetic theory $T$
defines a function $f$ when there is a formula $\fone$
in the language of $T$ such that $f$ satisfies $\fone(x,f(x))$
for any $x$ and $T\vdash (\forall x)(\exists !y) \fone (x,y)$.
%
The constructive proof of $(\forall x)(\exists y)\fone (x,y)$
also provides an algorithm to compute $f$.
%
So, the given procedure is effectively computable 
but not necessarily \emph{feasible}, that is 
\emph{computable in polynomial time}. 
%
Due to his bounded theories, Buss was able to arithmetically
characterize functions computable with given resource bound,
thus to characterize interesting complexity classes.
%
%
 \small
 \begin{figure}[h!]\label{fig:schema2}
\begin{center}
\framebox{
\parbox[t][2.6cm]{5cm}{
\footnotesize{

 \begin{center}
 \begin{tikzpicture}[node distance=2cm]
\node at (0,2) (a) {$\PTCA$}; %{Existential Preservation of Validity through $\Dec$};
\node at (-1.6,0.7) (b) {$\Sigma^b_1$-NIA}; 
\node at (1.6,0.7) (c) {$\FP$};

    \draw[<->,thick] (a) to [bend right=20] (b);
    \draw[<->,thick] (b) to [bend right=20] (c);
    \draw[<->,thick] (c) to [bend right=20] (a);

    %child {node {child 1}}
    %child {node {child 2}};
   %
\end{tikzpicture} 
 \end{center}
  }}}
\caption{Ferreira's Proof Schema~\cite{Ferreira88}}
\end{center}
\end{figure}  
\normalsize
%
%
%
%
%
\paragraph{Language.}
The language of Buss' fragments extends that of $\PA$
with three special predicate symbols:
$\llcorner \frac{1}{2} \cdot \lrcorner$ which divides for two
and round down the argument,
$|\cdot|$ 
returning the length of the binary representation the argument,
and the Nelson's function $\#$, such that $x\#y=2^{|x|\cdot |y|}$.
%
%The growth rate of $\#$ (is the same growth as that of the $\omega_1$-function and) is what needed to define functions in $\PH$.
%
%
In the language of $\BA$, standard quantifiers  are called \emph{unbounded}, 
while quantifiers of the form
$(\forall x\leq t)$ or $(\exists x\leq t)$ are called \emph{bounded}
and are such that $(\forall x\leq t)\fone$ is an shorthand
of  $(\forall x)(x\leq t\rightarrow \fone)$, and 
$(\exists x)\fone$ abbreviates
$(\exists x)(x\leq t\wedge \fone)$.\footnote{Otherwise, the
 syntax can be expanded so to directly include them.
In this case the calculus must be extended accordingly.}
%
A special kind of bounded quantifiers are \emph{sharply bounded}
ones, namely $(\forall x\leq |t|)$ and $(\exists x\leq |t|)$.
%
Bounded formulas (converted into PNF) are classified in a hierarchy of classes,
$\Sigma^b_k$ and $\Pi^b_k$, 
by counting alternations of bounded quantifiers
(ignoring sharply ones).







%%%
%%%
%%% LONG VERSION
\longv{
\begin{defn}
The set $\Delta^b_0=\Sigma^b_0=\Pi^b_0$
is equal to the set of formulas in which all
quantifiers are sharply bounded.
%
For $i\ge 1$, the sets $\Sigma^b_i,\Pi^b_i$
are inductively defined by the following conditions:
\begin{itemize}
\itemsep0em
\item If $\fone,\ftwo$ are $\Sigma^b_i$-formulas,
then $\fone\vee \ftwo$ and $\fone \wedge \ftwo$
are $\Sigma^b_i$-formulas.
If $\fone$ is a $\Pi^b_i$-formula and $\ftwo$
a $\Sigma^b_i$-formula, then $\fone \rightarrow \ftwo$,
and $\neg \fone$ are $\Sigma^b_i$-formulas.

\item if $\fone$ is a $\Pi^b_{i-1}$-formula,
then $(\exists x \leq t) \fone$ is a $\Sigma^b_i$-formula.

\item if $\fone$ is a $\Sigma^b_i$-formula
and $t$ a term,
then $(\forall x\leq |t|)\fone$ is a $\Sigma^b_i$-formula

\item if $\fone$ is a $\Sigma^b_i$-formula
and $t$ a term, then $(\exists x\leq t)\fone$
is a $\Sigma^b_i$-formula.
\end{itemize}
The four inductive conditions defining $\Pi^p_i$
are dual to the given ones.
\end{defn}
}





%%% DEFINITION BOUNDED FORMULAS
\longv{
\begin{defn}
The following sets of formulas
are defined by induction on the complexity of formulas:
\begin{enumerate}
\itemsep0em
\item $\Pi^b_0=\Sigma^b_0=\Delta_0^b$ is
the set of formulas the quantifiers of which 
are sharply bounded.

\item $\Sigma^b_{k+1}$ is defined inductively by
\begin{enumerate}
\itemsep0em
\item $\Sigma^b_{k+1}\subseteq \Pi^b_k$
\item if $\fone\in\Sigma^b_{k+1}$, then $(\exists x\leq t)\fone,
(\forall x\leq |t|) \fone \in \Sigma^b_{k+1}$
\item if $\fone,\ftwo\in \Sigma^b_{k+1}$, then
$\fone\wedge \ftwo, \fone \vee \ftwo\in \Sigma^b_{k+1}$
\item if $\fone \in \Sigma^b_{k+1}$
and $\ftwo\in \Pi^b_{k+1}$, then $\neg \ftwo,
\ftwo \rightarrow \fone \in \Sigma^b_{k+1}$.
\end{enumerate}
\item Similarly for $\Pi^b_{k+1}$.
\end{enumerate}
\end{defn}}









\paragraph{Axiomatization.}
Bounded theories are then defined by adding 32 basic 
axioms~\cite[pp. 30-31]{Buss86} to the ones for
$\PA$ and restricting  the induction schema.
%
%
%
%Basic axioms are sufficient to define the simple properties relating the function and predicate symbols of $\BA$.
%
Buss himself noticed that there is a certain amount of flexibility
in the choice of basic axioms and the ones he introduced
in his thesis are not optimal~\cite[p. 101]{Buss98}.
%
Alternative sets were proposed for example by Cook and Urquhart~\cite{CookUrquhart}
and Buss and Ignjatovi\'c~\cite{BussIgnjatovic}.\footnote{For further details, see~\cite{Buss98}}
In particular, Buss introduced the class 
$\textsf{\textbf{S}}^i_2$ as axiomatized by basic axioms plus $\Sigma^b_i$-PIND:
$$
\fone(x) \wedge (\forall x)(\fone (\llcorner \frac{1}{2}x\lrcorner)
\rightarrow \fone(x)) \rightarrow (\forall x)\fone (x),
$$
where $\fone$ is a $\Sigma^b_i$-formula,
while
$\textsf{\textbf{T}}^i_2$ are defined by the same set of basic 
axioms together with the induction schema $\Sigma^b_i$-IND,
$$
\fone(\zzero) \wedge (\forall x)(\fone(x) \rightarrow
\fone(\suc(x)) \rightarrow (\forall x)\fone(x),
$$
where $\fone$ is a $\Sigma^b_i$-formula.






%%%%% PARAGRAPH
%%%%% Relating S^1_2 and poly-time computable functions
\paragraph{Relating $\BussS$ and poly-time computable functions.}
The main result of Buss' Thesis is the proof that these arithmetic theories actually provide a logical characterization of complexity classes
in $\PH$.
%
In particular, he proved that poly-time computable functions
are $\Sigma^b_1$-definable in $\BussS$~\cite[Cor. 8, p. 99]{Buss86}.
%
On the one hand, 
a function is poly-time computable when there is a TM $\TM$
and a polynomial $p(n)$ such that $\TM$ computes the given function
and runs in time smaller or equal than $p(n)$, for any input of length
$n$.
%
In 1964, this notion was made precise by Cobham in the form of
a function algebra~\cite{Cobham}, on which Buss' proof relies.\footnote{Buss also noticed that a proof ``directly'' based on the machine definition is also possible.}
On the other, 
a function is $\Sigma^b_1$-definable in $\BussS$ %(or in a given theory $T$) 
when there is a $\Sigma^b_1$-formula $\fone$ such that 
conditions above hold.
%
The link between complexity of computing and 
quantified formulas is then established in two main steps:
 \footnotesize
 \begin{center}
 \begin{tikzpicture}[node distance=2cm]
%\node at (0,2) (a) {$\Sigma^b_1$-representability in $\RS$}; %{Existential Preservation of Validity through $\Dec$};
\node at (7,0) (a) {$\Sigma^b_1$-representability in $\BussS$~\cite{Buss86}}; 
\node at (2,0) (b) {Class $\mathcal{FP}$~\cite{Cobham}};
\node at (4.5,1) {\textcolor{gray}{\scriptsize{witness theorem}}};
\node at (4.5,-1) {\textcolor{gray}{\scriptsize{bootstrapping}}};

    \draw[->,thick,gray] (a) to [bend right=25] (b);
    \draw[->,thick,gray] (b) to [bend right=25] (a);
    %\draw[<->,thick,dotted,gray] (c) to [bend right=20] (a);

    %child {node {child 1}}
    %child {node {child 2}};
   %
\end{tikzpicture} 
\end{center}
\normalsize
\noindent
That every poly-time function is $\Sigma^b_1$-definable
in $\BussS$ is proved due to the so-called \emph{bootstrapping}, 
that is a series of coding functions was introduced.
%
The proof of the converse direction is more difficult.
Buss presented a sequent calculus, extending 
$\mathbf{LK}$ with rules
for limited induction and bounded quantifiers.
Then, due to cut elimination, he proved the ``witness'' theorem,
showing that proofs in this calculus contain explicit 
algorithms to compute the output of the function from the input
\emph{in polynomial time}.







\subsection{Ferreira's Bounded Arithmetic}
In~\cite{Ferreira88,Ferreira90}, Ferreira introduced
a ``(supposedly) more natural''~\cite[p. 2]{Ferreira90} 
bounded theory defined in a word language,
instead of the standard language of arithmetic $\mathcal{L}_{\Nat}$.
%
This arithmetic characterizes poly-time 
computable functions – this time defined over
strings – and, indeed, can interpret Buss' 
$\BussS$~\cite{FerreiraOitavem}.
%
For clarity's sake, we sum up its salient aspects
following notation and axiomatization 
by~\cite{FerreiraOitavem}, which is slightly different from~\cite{Ferreira88,Ferreira90} in the surface 
but essentially equivalent.




\paragraph{The Function Algebra $\PTCA$.}
Ferreira defined an algebra of functions \emph{over strings}
$\PTCA$
(poly-time computable arithmetic) analogous
to Cobham's one but made of:
%
%
%
\begin{itemize}
\itemsep0em
\item initial functions:
\begin{itemize}
\itemsep0em
\item $E_{\mathcal{F}}(x)=\emptyset$
\item $P_{\mathcal{F}}^{n,i}(x_1,\dots, x_n)=x_i$, with $1\leq i\leq n$
\item $C^b_{\mathcal{F}}(x)=x\bool$, where if $b=1$, then $\bool=\one$ and
if $b=0$, then $\bool=\zero$
\item \begin{align*}
Q_{\mathcal{F}}(x,y) =\one &\leftrightarrow x\subseteq y \\ 
Q_{\mathcal{F}}(x,y) = \zero &\vee Q_{\mathcal{F}}(x,y)=\one
\end{align*}

\end{itemize}

\item functions obtained by:
\begin{itemize}
\itemsep0em

\item composition, i.e. $f$ is obtained from $g,h_1,\dots,h_k$
as $f=(x_1,\dots, x_n)=g(h_1(x_1,\dots, x_n),\dots, h_k(x_1,\dots, x_n))$

\item bounded iteration, i.e. $f$ is obtained from $g,h_0,h_1$ as,
\begin{align*}
f(x_1,\dots, x_n,\emptyset) &= g(x_1,\dots, x_n) \\
f(x_1,\dots, x_n,y\bool) &= 
h_b(x_1,\dots, x_n,y,f(x_1,\dots, x_n,y))|_{t(x_1,\dots, x_n,y)}
\end{align*}
where $t$ is a term called \emph{bound} and $\cdot |_{\cdot}$
denote truncation.
\end{itemize}
\end{itemize}






\paragraph{The Word Language $\mathcal{L}_{\mathbb{W}}$.}
As anticipated, Ferreira's theory is defined in a word
language $\mathcal{L}_{\mathbb{W}}$, which is basically
a first-order language with equality endowed with 
three constants $\epsilon,\zzero,\one$,
two function symbols $\conc, \times$
and a relation symbol $\subseteq$.\footnote{Observe that
Ferreira used different symbols for the empty
string and for concatenation.}
Interpretation is as predictable:
$\epsilon$ denotes the empty
word, $\zzero$ and $\oone$ 
the bits $\zero$
and $\one$ (resp.),
$\conc$ word concatenation,
$\times$ the binary product (i.e.~$x\times y=
x\conc\dots \conc x$, $|y|$-times),
and $\subseteq$ the \emph{initial} subword relation.
%
%
\emph{Bounded quantifiers} in $\mathcal{L}_{\mathbb{W}}$
are of the form $\forall x\preceq t$ and $\exists x\preceq t$
(with $t$ term),
where $x\preceq t$ intuitively means that the length
of $x$ is smaller or equal than that of $t$.
Bounded-quantified formulas $(\forall x\preceq t)\fone$
and $(\exists x\preceq t)\fone$
abbreviates respectively $(\forall x)(\one\times x \subseteq \one \times t
\rightarrow \fone)$
and $(\exists x)(\one\times x\subseteq \one \times t
\wedge \fone)$.
%
\emph{Subword quantifiers} are of the form
$\forall x\subseteq^* t$ and $\exists x\subseteq^* t$, 
so defined that $(\forall x\subseteq^* t)\fone$
is a shorthand for $(\forall)(\exists w
\subseteq t(wx\subseteq t)\rightarrow \fone)$
and $(\exists x\subseteq^* t)\fone$
for $(\exists x)(\exists w\subseteq t(wx\subseteq t)\wedge
\fone)$.


\paragraph{The Theory $\Sigma^b_1$-NIA.}
Then, $\Sigma^b_1$-NIA is a first-order theory
in $\mathcal{L}_{\mathbb{W}}$
defined by the following axioms:\footnote{Again,
the name $\Sigma^b_1$-NIA is not original by~\cite{Ferreira88},
but was introduced in~\cite{FerreiraOitavem}.}
%
%
\begin{itemize}
\itemsep0em
\item Basic axioms:
\begin{center}
$x \epsilon = x$ \ \ \  \ \ \
$x(y\bbool) = (xy)\bbool$  \ \ \ \ \ \ \
%
$x \times \epsilon = \epsilon$ \ \ \  \ \ \ 
$x\times y\bbool = (x\times y)x$ \\
%
$x\subseteq \epsilon \leftrightarrow x=\epsilon$
\ \ \  \ \ \  
$x\subseteq y\bbool \leftrightarrow x\subseteq y \vee x=y\bbool$ \\ 
%
$x\bbool = y\bbool \rightarrow x=y$  \ \ \ \ \ \ 
%
$x\zzero \neq y \oone$ \ \ \ \ \ \  $x\bbool \neq \epsilon.$
\end{center}

\item Axiom schema for induction on notation:
$$
\fone(\epsilon) \wedge (\forall x)(\fone(x) \rightarrow \fone(x\zero)
\wedge \fone(x\one)) \rightarrow (\forall x)\fone (x),
$$
where $\fone$ is a $\Sigma^b_1$-formula in $\mathcal{L}_{\mathbb{W}}$.
%that is of the form $(\exists x)(x\preceq t(\vec{z})\wedge \fone(\vec{z},x))$, where $\fone$ is a sw.q. formula, i.e. $\fone$ belongs to the smallest class of formulas of $\mathcal{L}_{\mathbb{W}}$ containing atomic formulas and closed under Boolean operations and subword quantification.  
\end{itemize}













\longv{What is meant by talking of an \emph{effective} computational procedure?
%
The core idea is that an effective computation involves (1) executing an \emph{algorithm} which (2) successfully \emph{terminates}.
%
If executing an algorithm is computing a total function,  then the procedure must \emph{terminate} in a finite number of steps for every input, and produce the right sort of output.
%
Observe that it it not part of the very idea of an algorithm that its execution always terminates.
% An algorithm might compute partial functions.
% Informally, the idea is that an effective computable function is one that a computer could compute.
By Kleene's theorem, every partial recursive function $f$ can be written as $f(\vec{n})=l(\mu y[t_f(\vec{n},y)=0])$, where $l$ and $t_f$ are primitive recursive. 
%
The function $t_f$ describes a particular algorithm computing $f$.
%%
Termination of this algorithm can be expressed by a formula of the form
$$
(\forall \vec{x})(\exists y)t_f(\vec{x},y)=0.
$$
If this formula has a proof, one can say that the function is provably total.
%
Define Kleene's $T$ predicate:
$$
T(k,\vec{n},m) \ \ \ \text{ iff } \ \ \ \TM_k \text{halts on input } \vec{n}
\text{ in } r(m) \text{ steps without output } l(m).
$$
which is primitive recursive. 
%
Let $f$ be a partial function computed by $\TM_k$.
%
Then, the characteristic function of $T$ is
$$
t_f(\vec{n},m)=0 \ \ \ \text{ iff } \ \ \ \TM_k \text{ halts on input }
\vec{n} \text{ in } r(m) \text{ steps with output } l(m).
$$
and is primitive recursive.
%
By Kleene's theorem of normal form, every partial recursive function $f$ can be written as $l(\mu y[t_f(\vec{n},y)=0])$, where $t_f$ and $l$ are primitive recursive functions. 
%
A recursive function $f$ is \emph{provably total} in a theory $T$ when
$$
T \vdash (\forall \vec{x})(\exists y)(t_f(\vec{x},y)=0.
$$
$$
\frac{\text{totality of functions}}{\text{termination}}
= \frac{x}{\text{probabilistic termination}}
$$}






